PCC: Re-architecting Congestion Control for Consistent High Performance

TCP and its variants have suffered from surprisingly poor performance for decades. We argue the TCP family has little hope to achieve consistent high performance due to a fundamental architectural deficiency: hardwiring packet-level events to control responses without understanding the real performance result of its actions. We propose Performance-oriented Congestion Control (PCC), a new congestion control architecture in which each sender continuously observes the connection between its actions and empirically experienced performance, enabling it to consistently adopt actions that result in high performance. We prove that PCC converges to a stable and fair equilibrium. Across many real-world and challenging environments, PCC shows consistent and often 10x performance improvement, with better fairness and stability than TCP. PCC requires no router hardware support or new packet format.

==> keyidea.tex <==
\subsection{The Key Idea}

Suppose flow $f$ is sending a stream of data at some rate and a packet is lost.  How should it react?  Should it slow the sending rate, or increase, and by how much? Or leave the rate unchanged?  This is a difficult question to answer because real networks are complex.  A single loss might be the result of \emph{many} possible underlying network scenarios. To pick a few:
\begin{itemize}
\vspace{-3mm}
	\item $f$ may be responsible for most of congestion.  Then, it should decrease its rate.
\vspace{-3mm}
	\item $f$ might traverse a shallow buffer on a high-BDP link, with the loss due to bad luck in statistical multiplexing rather than high link utilization.  Then, backing off a little is sufficient.
\vspace{-3mm}    
    \item There may be a higher-rate competing flow. Then, $f$ should maintain its rate and let the other back off.
\vspace{-6mm}	
\item There may be random non-congestion loss somewhere along the path.  Then, $f$ should maintain or increase its rate.
\end{itemize}
\vspace{-2mm}

Clasically, TCP assumes a packet loss indicates non-negligible congestion, and that halving its rate will improve network conditions.  However, this assumption is false and will degrade performance in three of the four scenarios above.  Fundamentally, picking an optimal \emph{predefined and hardwired} control response is hard because for the same packet-level events, a control response optimal under one network scenario can decimate performance in even a slightly different scenario.  The approach taken by a large number of TCP variants is to design more sophisticated packet-level events and control actions; but this approach does not solve the fundamental problem, because \emph{they still hardwire predetermined events to predetermined control responses}, thus inevitably embedding unreliable assumptions about the network. The real network can have complexity beyond what any hardwired mapping can model, as discussed in~\S\ref{sec:intro}, and when the unreliable assumptions are violated, performance can degrade severely. For example, TCP Illinois~\cite{illinois} uses both loss and delay to form a complicated packet-level event-control mapping, but its throughput catastrophically collapses with even a tiny amount of random loss, or when the network is dynamically changing (\S\ref{sec:eval}). More examples are in \S\ref{sec:rel}.


%For example, TCP Illinois~\cite{illinois}, the Linux default since kernel 2.6.19, uses a cubic window expansion algorithm to mitigate the problem of slow recovery in high-BDP links but its throughput catastrophically collapses with even a tiny amount of random loss (\S\ref{sec:eval}). More examples are in \S\ref{sec:rel}.

Most unfortunately, if some control actions are indeed harming performance, TCP can still mechanically ``jump off the cliff'' again and again, because it does not notice the control action's actual effect on performance.

%TCP's assumptions will often be wrong, so it takes a control action that worsens performance, and indeed may continue taking this harmful action repeatedly.

But that observation points towards a solution.  Could we design a control algorithm that directly understand whether its control actions actually improve performance or not?

Conceptually, no matter how complex the network is, if a sender can directly measure that rate $r_1$ results in better performance than rate $r_2$, it has some evidence that $r_1$ is better than sending at $r_2$ --- at least for this one sender. This example illustrates the key design rationale behind \textbf{Performance-oriented Congestion Control} (PCC): we make control decisions based on \emph{empirical evidence pairing actions with directly observed performance results}.

PCC's control action is its choice of sending rate. PCC divides time into continuous equal time periods, called \emph{monitor intervals}, whose length is normally one to two RTTs. In each monitor interval, PCC tests an action: it picks a sending rate, say $r$, and sends data at this rate through the interval. After about an RTT, the sender will see selective ACKs (SACK) from the receiver, just like TCP. However, it does not trigger any predefined control response. Instead, PCC aggregates these SACKs into meaningful performance metrics including throughput, loss rate and latency. These performance metrics are combined to a numerical utility value, say $u$, via a \emph{utility function}. The utility function can be customized for different data transmission objectives (discussed in ~\S\ref{?}), but for now the reader can assume the objective of ``high throughput and low loss rate'', such as $u=T-L$ (where $T=$ throughput and $L=$ loss rate) which will capture the main insights of PCC. The end result is that PCC knows when it sent at rate $r$, it got utility of $u$.

The preceding describes a single ``experiment'' through which PCC associates a specific \emph{action} with an observed \emph{resulting utility}.  PCC runs these experiments continuously, comparing the utility of different sending rates so it can track the optimal action over time. More specifically, PCC runs a gradient-ascent online learning algorithm. When starting at rate $r$, it tests rate $(1+\eps)r$ and rate $(1-\eps)r$, and moves in the direction (higher or lower rate) that empirically results in higher utility.  It then continues in this direction as long as utility continues increasing.  If utility falls, it returns to a decision-making state where it again tests both higher and lower rates to determine which produces higher utility.

Note that PCC does not send occasional probes or use throwaway data for measurements.  It observes the results of its actual control decisions on the application's real data, so that every byte of data is part of a measurement.

\parheading{We now return to the example} of the beginning of this section.  Suppose PCC is testing rate $100$~Mbps in a particular interval, and will test $105$ Mbps in the following interval.  If it encounters a packet loss in the first interval, will PCC increase or decrease?  In fact, there is no specific event in a single interval that will always cause PCC to increase or decrease its rate.  Instead, PCC will calculate the utility value for each of these two intervals, and move in the direction of higher utility.  For example:
\begin{itemize}
	\item If the network is congested as a result of this flow, then it is likely that sending at $100$~Mbps will have similar throughput and lower loss rate, resulting in higher utility. PCC will decrease its rate.
	\item If the network is experiencing random loss, PCC is likely to find that the period with rate $105$~Mbps has similar loss rate and slightly higher throughput, resulting in higher utility.  PCC will therefore increase its rate despite the packet loss.
\end{itemize}

Throughout this process, PCC makes no assumptions about the underlying network conditions. It treats the network as a black box, observing which actions empirically produce higher utility and therefore achieving consistent high performance.

\parheading{Decisions with noisy measurements.}  PCC's experiments on the live network will tend to move its rate in the direction that empirically improves utility.  But it may also make some incorrect decisions.  In the example above, if the loss is random non-congestion loss, it may randomly occur that loss is substantially higher when PCC tests rate $105$~Mbps, causing it to pick the lower rate.  Alternately, if the loss is primarily due to congestion from this sender, unpredictable external events (perhaps another sender arriving with a large initial rate while PCC is testing rate $100$ Mbps) might cause rate $105$~Mbps to have higher throughput and lower loss rate.  More generally, the network might be changing over time for reasons unrelated to the sender's action.  This adds noise to the decision process: PCC will on average move in the right direction, but may make some unlucky errors.

We improve PCC's decisions with \textbf{multiple randomized controlled trials (RCTs)}. Rather than running two tests (one each at $100$ and $105$~Mbps), we conduct four in randomized order---e.g. perhaps $(100,105,105,100)$.  PCC only picks a particular rate as the winner if utility is higher in \emph{both} trials with that rate.  This produces increased confidence in a causal connection between PCC's action and the observed utility.  As we will see, without RCTs, PCC already offers a dramatic improvement in performance and stability compared with TCP, but RCTs further reduce rate variance by up to \fixme{$40$\%}.  Although it might seem that RCTs will double convergence time, this is not the case because they let PCC make \emph{better} decisions; overall, RCTs improve the stability/convergence-speed tradeoff space.

\parheading{Many issues remain.}  We next delve into fairness, convergence, and choice of utility function; deployment of PCC; and detailed description of the mechanism sketched above.



%Remy~\cite{remy, learnabilitytcp} pushes TCP's architecture perhaps as far as it can go, by simulating possible protocols to find which hardwired controls tend to perform well in given scenarios.  But even Remy's algorithmically-designed hardwired control protocols fail to adapt to varying number of senders and other parameters \fixme{make that statement stronger}.

%- TCP's assumptions will often be wrong, so it takes a control action that worsens performance, and indeed may continue taking this harmful action repeatedly.

%In fact, actual production network can have complexity beyond the assumptions embedded in any hardwired mapping: old and unreliable routers, failing physical wires, instability of routing paths, AQMs, virtualization layers, software routers, rate shaping at boarder gateways and middle boxes like firewalls, VPN, packet inspectors and load balancers. All these factors add so much uncertainty that can almost surely violates any TCP-like hardwired mapping's relatively simplistic assumptions about networks and more importantly, \emph{make it impossible to build a hardwired mapping having all these factors considered}.

%Before moving to an example, we clarify two \textbf{\emph{common misunderstandings}} of PCC's mechanism: \emph{Mis. 1.} PCC sends for one monitor interval and stops sending to wait for feedbacks. \emph{Expl. 1.} PCC continuously sends data without waiting. If at the beginning of a monitor interval, PCC's control algorithm does not change sending rate, PCC will just continue to send at the previous monitor interval's sending rate. \emph{Mis. 2.} After PCC makes a control decision, it will just send at that rate for a long time with no more measuring. \emph{Expl. 2.} PCC never stops actively monitoring performance. PCC is either in the state of deciding which direction it should change the sending rate or in the state of changing rate continuously towards a certain direction. Both require continuous monitoring of utility. This continuous experimenting makes PCC agile to network change and resilient to noisy measurement.

